Finite Sample Confidence Regions for Linear Regression Parameters Using Arbitrary Predictors

We explore a novel methodology for constructing confidence regions for parameters of linear models, using predictions from any arbitrary predictor. Our framework requires minimal assumptions on the noise and can be extended to functions deviating from strict linearity up to some adjustable threshold, thereby accommodating a comprehensive and pragmatically relevant set of functions. The derived confidence regions can be cast as constraints within a Mixed Integer Linear Programming framework, enabling optimisation of linear objectives. This representation enables robust optimization and the extraction of confidence intervals for specific parameter coordinates. Unlike previous methods, the confidence region can be empty, which can be used for hypothesis testing. Finally, we validate the empirical applicability of our method on synthetic data.

==> subfiles/conformal_based.tex <==

\section{From Prediction Set to Confidence Set}

(Assume basic notations and assumptions have been introduced above).

\subsection{Confidence Set From a Single Test Point}

The key idea of this work is to leverage the prediction sets provided by a (potentially black-box) CP algorithm to infer confidence sets on the parameters of a parametric model. While these confidence sets may take complex forms, we show in section \ref{sec:application} how they can be leveraged within tractable optimization problems to be applied to e.g. interpretability and hypothesis testing. 

let us consider the following linear model parameterized by $\theta$:
\begin{equation}
    y = \theta^T x + \epsilon
\end{equation}
Where $x$ is the observed variable, $y$ is the regression target, and $\epsilon$ is the noise. Notably, we do not assume knowledge of the functional form of the noise, nor do we assume its independence wrt the observed variable $x$. Instead, we make the following assumption:
\begin{assumption}
\label{assumption:noise}
    There exists $u>0$ such that $\forall x\in X, \mathbb{P}(\epsilon>0\mid x)\leq 1-u$ and $\mathbb{P}(\epsilon<0\mid x)\leq 1-u$.
\end{assumption}
Intuitively, the noise should not be too unbalanced anywhere on $X$. In particular, if $\epsilon$ has median $0$ everywhere, then Assumption \ref{assumption:noise} is verified with $u=\frac{1}{2}$. This assumption is very weak compared to prior works which typically assume Gaussian noise with constant variance over $X$, and it captures a much wider set of models, such as linear models with multiplicative noise.
\begin{remark}
    Let $\eta$ be a random noise verifying Assumption \ref{assumption:noise} for some $u>0$. Then, the linear model with multiplicative noise $y=\theta^T x (1+\eta)$ can be cast as $y=\theta^T x + \epsilon$ with $\epsilon=\eta\theta^T x$. In this case, the distribution of $\epsilon$ also verifies Assumption \ref{assumption:noise} with the same $u$.
\end{remark}
\textcolor{red}{do we need to include proof or is it trivial enough ?}

We now assume access to a black-box CP Algorithm $\mathcal{A}$ which observes data $X,Y = (x_i,y_i)_{i=1,\dots,n}$ and a test point $x_{n+1}$, and outputs a prediction interval $S_{X,Y}(x_{n+1})$ verifying for some $\alpha>0$ the conformity guarantee: 
\begin{equation}
\label{eq:conformity}
    \mathbb{P}_{\mathcal{D}_{n+1}\sim \mathcal{P}}[y_{n+1}\in S_{X,Y}(x_{n+1})]\geq 1-\alpha. 
\end{equation}

$$ \mathcal{D}_{n+1} = \{(x_1,y_1), \ldots,(x_{n+1},y_{n+1})\} $$

\textbf{Maybe let's write it for a single variable first}

\begin{prop}
Let $\varepsilon$ be any noise, we assume an additive model 
$$ y = f_{\theta^\star}(x) + \epsilon $$
Then it holds
$$
\frac{\mathbb{P}(y \in [a, b]) - \max( \mathbb{P}(\varepsilon > 0), \mathbb{P}(\varepsilon < 0))}{1 -  \max( \mathbb{P}(\varepsilon > 0), \mathbb{P}(\varepsilon < 0))} \leq  \mathbb{P}( f_{\theta^\star}(x) \in [a, b])
$$
\end{prop}


If the interval $[a, b]$ covers $y$ with probability larger than $1 - \alpha$ and the noise satisfies
$$ \max( \mathbb{P}(\varepsilon > 0), \mathbb{P}(\varepsilon < 0)) \leq 1 - u, $$
it holds
% 
\begin{align*}
    \mathbb{P}(f_{\theta^\star}(x) \in[a,b]) \geq \frac{1-\alpha-(1-u)}{1 -(1 - u)}=1-\frac{\alpha}{u}
\end{align*}

Now for an iid sample $y_i = f_{\theta^\star}(x_i) + \epsilon_i$, we have
% $$
% \frac{\mathbb{P}^{n+1}(y_{n+1} \in [a_{n+1}, b_{n+1}]) - \max(\mathbb{P}^{n+1}(\varepsilon_{n+1} > 0), \mathbb{P}(\varepsilon_{n+1} < 0))}{1 -  \max( \mathbb{P}^{n+1}(\varepsilon_{n+1} > 0), \mathbb{P}^{n+1}(\varepsilon_{n+1} < 0))} \leq  \mathbb{P}^{n+1}( f_{\theta^\star}(x_{n+1}) \in [a_{n+1}, b_{n+1}])
% $$

$$ \mathbb{P}^{n+1}( f_{\theta^\star}(x_{n+1}) \in [a_{n+1}, b_{n+1}]) \geq  1-\frac{\alpha}{u} $$

Wait, this already is nice. we have a confidence on the ground-truth prediction $y^\star$ (and for this, no inversion is needed. meaning that $f$ can be arbitrarily complicated, we do not care ... we might be able to get nice application from this alone) ...

\paragraph{Hypothesis testing}
Given an input $x$ we want to test

$$ H_0: y^\star(x) \in \mathcal{Y}_0 \text{ or not} $$

it suffices to check if the intersection $\mathcal{Y}_0  \cap [a(x), b(x)]$ is empty.

\textbf{However, it is unclear of to get the constant $u$ in practice ... maybe not a big deal}

\begin{lemma}
$$ 1 - \alpha - \mathbb{P}(\varepsilon \notin [\delta_{-}, \delta_{+}]) \leq \mathbb{P}(f_{\theta^\star}(x) \in [a - \delta_{+}, b - \delta_{-}] ) $$
\end{lemma}


As such, a confidence set on the noise ie $\mathbb{P}(\varepsilon \notin [\delta_{-}, \delta_{+}]) \leq \alpha$ results in a factor $2$ loss in the coverage.




We can now start inferring confidence sets on $\theta$ from $\mathcal{A}$:
\begin{prop}
\label{prop:1}
    Under the same notations,
    \begin{equation}
    \label{eq:prop2}
        \mathbb{P}_{(x_1,y_1),\dots,(x_{n+1},y_{n+1})\sim \mathcal{P}}[\theta^T x_{n+1}\in S_{X,Y}(x_{n+1})]\geq 1-\frac{\alpha}{u}.
    \end{equation}
\end{prop}

% \begin{proof}
%     Let $E$ denote the event $y_{n+1}\in [a,b]:=S_{X,Y}(x_{n+1})$. Within the scope of this proof, all probabilities are considered over the distribution of $x_1,y_1,\dots,x_{n+1},y_{n+1}$.

%     \textcolor{red}{Notation issue here, I'm using $x$ instead of $x_{n+1}$ because otherwise the equations are too long...}

%     \begin{align*}
%         \mathbb{P}(E)&=\mathbb{P}(E\mid \theta^T x\in [a,b])\mathbb{P}(\theta^T x\in[a,b]) + \mathbb{P}(E\mid \theta^T x>b)\mathbb{P}(\theta^T x>b) + \mathbb{P}(E\mid \theta^T x < a)\mathbb{P}(\theta^T x<a])\\
%         &\leq \mathbb{P}(\theta^T x\in[a,b]) + (1-u)\mathbb{P}(\theta^T x>b) + (1-u)\mathbb{P}(\theta^T x<a)\\
%         &= \mathbb{P}(\theta^T x\in[a,b]) + (1-u)\mathbb{P}(\theta^T x\not \in[a,b])\\
%         &= 1-u+u\mathbb{P}(\theta^T x\in[a,b])
%     \end{align*}

%     Since Equation \eqref{eq:conformity} stipulates that $\mathbb{P}(E)\geq 1-\alpha$, we finally get
%     \begin{align*}
%         \mathbb{P}(\theta^T x\in[a,b])\geq \frac{1-\alpha-1+u}{u}=1-\frac{\alpha}{u}
%     \end{align*}
% \end{proof}

Proposition \ref{prop:1} can be seen as a conformity guarantee over the confidence set $S^{-1}_{X,Y}(x_{n+1}):=\{\theta\in\Theta:\theta^T x_{n+1}\in S_{X,Y}(x_{n+1})\}$. Indeed, it implies $\mathbb{P}_{x_1,y_1,\dots,x_{n+1},y_{n+1}}(\theta\in S_{X,Y}^{-1}(x_{n+1}))\geq 1-\frac{\alpha}{u}$.
$S^{-1}_{X,Y}(x_{n+1})$ is the space contained between two hyperplanes, and possess limited information : for instance it is necessarily unbounded. 

Therefore, we now seek to shrink our confidence set by combining the information from multiple test points.

The probability of an intersection can be easily bounded as
% 
\begin{align*}
\mathbb{P}(\theta \in \cap_{k=1}^{m} \Theta_k) &= 
1 - \mathbb{P}(\theta \notin \cap_{k=1}^{m} \Theta_k) \\
&= 1 - \mathbb{P}(\theta \in \cup_{k=1}^{m} \Theta_{k}^{c}) \\
&\geq 1 - \sum_{k=1}^{m} \mathbb{P}(\theta \in \Theta_{k}^{c}).
\end{align*}
% 
Hence $\mathbb{P}(\theta \in \Theta_{k}) \geq 1 - \alpha_k$ implies that $\mathbb{P}(\theta \in \Theta_{k}^{c}) = 1 - \mathbb{P}(\theta \in \Theta_{k}) \leq 1 - (1 - \alpha_k) = \alpha_k$ and
% 
$$ \mathbb{P}(\theta \in \cap_{k=1}^{m} \Theta_k) \geq 1 - \sum_{k=1}^{m} \alpha_k $$




\subsection{Hard Intersection of Confidence Sets}
\label{subsec:hard_intersect}

The most straightforward approach to combining confidence sets from different test points is to simply intersect them. Let us assume we are now given $k$ test points $x_{n+1},\dots,x_{n+k}$, and denote $E_k$ the event $\theta\in S_{X,Y}^{-1}(x_{n+k})$. We define our intersected confidence set as $S_{X,Y}^{-1}:=\bigcap_k S_{X,Y}^{-1}(x_{n+k})$. By construction $\theta\in S_{X,Y}^{-1}\Leftrightarrow \land_k E_k$, however the $E_k$ have a common dependence on $X,Y$, making the probability of $\land_k E_k$ not straightforward to compute. Luckily, Proposition \ref{prop:indep_is_worst_case} shows that full independence is the worst case scenario for the probability of $\land_k E_k$, allowing us to derive a simple conformity probability.

\begin{prop}
    \label{prop:indep_is_worst_case}
    Under the above setting,
    \begin{equation}
        \mathbb{P}_{x_1,y_1,\dots,x_{n+k},y_{n+k}}(\land_k E_k)\geq (1-\frac{\alpha}{u})^k
    \end{equation}
\end{prop}


Proposition \ref{prop:indep_is_worst_case} allows us to intersect confidence sets at the cost of significance level. When fixing $(1-\frac{\alpha}{u})^k$ and increasing $k$, this is equivalent to decreasing $\alpha$ and thus increasing the size of the $S^{-1}_{X,Y}(x_{n+k})$. This leads to the following tradeoff: increasing the number of test points implies to take an intersection over a larger number of sets, but simultaneously makes each of the sets larger.

The main limitation of this approach is the exponential dependence in $k$. Indeed, the CP algorithm may be unreliable or return unreasonably large prediction sets when setting $\alpha$ too low, which severely limits the number of test points that can realistically be used to compute the confidence set.

\subsection{Soft Intersection of Confidence Sets}
To alleviate the issue of the exponential dependence in $k$ when intersecting confidence sets, we now propose to only require $\theta$ to belong in at least $k$ of $m$ confidence sets, i.e., we consider the following confidence set:
\begin{equation}
    S_{k,m}^{-1}:=\bigcup_{\substack{\mathcal{I}\subseteq \{1,\dots,m\} \\ |\mathcal{I}|=k}}\left(\bigcap_{i\in\mathcal{I}}S_{X,Y}^{-1}(x_{n+i})\right).
\end{equation}
We consider two different settings: the full black-box setting in which we have no knowledge of how $\mathcal{A}$ constructs its prediction set, and the usual split CP setting in which the prediction sets are constructed by comparing the value of a conformity measure to the quantiles of that same conformity measure on a calibration set. By exploiting the structure of the prediction set, the second setting leads to better coverage guarantees than the general black-box setting.

\subsubsection{Fully black-box CP algorithm}

We wish to lower bound the coverage $\mathbb{P}(\theta\in S_{k,m}^{-1})$. Similarly to Section \ref{subsec:hard_intersect}, the common dependence of the $S_{X,Y}^{-1}(x_{n+1})$ on $X,Y$ impacts the coverage, and since we do not assume information on the structure of the prediction set, we resort to estimating the worst-case scenario. 

Given $Q(X,Y):=\mathbb{P}_x(\theta\in S_{X,Y}^{-1}(x)\mid X,Y)$, the probability to achieve at least $k$ successes out of $m$ trials is given by:
\begin{equation}
    \mathbb{P}(\theta\in S_{k,m}^{-1}\mid X,Y)=\sum_{i=k}^{m} \binom{m}{i}Q(X,Y)^i(1-Q(X,Y))^{m-i},
\end{equation}

Our goal is thus to find the infimum of $\mathbb{P}(\theta\in S^{-1}_{k,m})$ over all admissible $Q(X,Y)$, thus we want to solve:
\begin{equation}
\label{eq:worst-case}
\begin{aligned}
\min_{Q\in [0,1]^{dom(X)\times dom(Y)}} \quad & \int_{X,Y}\left(\sum_{i=k}^{m} \binom{m}{i}Q(X,Y)^i(1-Q(X,Y))^{m-i}\right)p(X,Y)\\
\textrm{s.t.} \quad & \int_{X,Y}Q(X,Y)p(X,Y)\geq 1-\frac{\alpha}{u}  \\
\end{aligned}
\end{equation}

A priori, this is an optimization problem over $Q$ which is infinite dimensional. However, we can leverage symmetries of the problem to considerably simplify it.

\begin{lemma}
    There exists $A\subseteq dom(X)\times dom(Y)$, and $1-\frac{\alpha}{u}\geq v \geq 0$ s.t. Problem (\ref{eq:worst-case}) admits at least one solution of the form $Q(X,Y)=v$ if $X,Y\in A$, else $Q(X,Y)=1$.
\end{lemma}

\begin{proof}
    Let the following optimization problem

\begin{equation}
\begin{aligned}
\min_{v,h\in [0,1]^3} \quad & h + (1-h)\left(\sum_{i=k}^{m} \binom{m}{i}v^i(1-v)^{m-i}\right)\\
\textrm{s.t.} \quad & h+(1-h)v\geq 1-\frac{\alpha}{u}  \\
\end{aligned}
\end{equation}
\end{proof}

\subsubsection{Rank-based CP algorithm}

In the split conformal prediction framework, $X,Y$ is split between a train set $X_{tr}, Y_{tr}$ and a calibration set $X_{cal}, Y_{cal}$ of size $n_{cal}$. A conformity score $C:dom(X)\times dom(Y)\rightarrow \mathbb{R}$ is then computed on all calibration pairs $x,y$, and the $\alpha$-quantile $q_\alpha(X_{cal},Y_{cal})$ of these validation conformity scores is inferred. Prediction sets for an input $x$ are subsequently defined as $\{y: C(x,y)\geq q_\alpha(X_{cal},Y_{cal})\}$.

This structure can be leveraged to derive conformal guarantees on the confidence set. Indeed,
\begin{equation}
\theta\in S_{X,Y}^{-1}(x)\Leftrightarrow C(x,\theta^T x)\geq q_{\alpha}(X_{cal},Y_{cal})
\end{equation}
Denote $\mathcal{C}_{cal}$ the distribution of $C(x,y)$ and $\mathcal{C}_{\theta}$ the distribution of $C(x,\theta^T x)$. 

\textcolor{red}{Find a rigorous formulation...}

$\theta\in S^{-1}_{k,m}$ iff at least $k$ of the $m$ variables $C(x_{n+i},\theta^T x_{n+i})$ which are iid (\textcolor{red}{for now, we'll see later for exchangeability}) with distribution $\mathcal{C}_\theta$, are below the $\alpha$-quantile of the $n_{cal}$ 
